Enhancing Automated Program Repair through Fine-tuning and Prompt Engineering

Sequence-to-sequence models have been used to transform erroneous programs into correct ones when trained with a large enough dataset. Some recent studies also demonstrated strong empirical evidence that code review could improve the program repair further. Large language models, trained with Natural Language (NL) and Programming Language (PL), can contain inherent knowledge of both. In this study, we investigate if this inherent knowledge of PL and NL can be utilized to improve automated program repair. We applied PLBART and CodeT5, two state-of-the-art language models that are pre-trained with both PL and NL, on two such natural language-based program repair datasets and found that the pre-trained language models fine-tuned with datasets containing both code review and subsequent code changes notably outperformed each of the previous models. With the advent of code generative models like Codex and GPT-3.5-Turbo, we also performed zero-shot and few-shots learning-based prompt engineering to assess their performance on these datasets. However, the practical application of using LLMs in the context of automated program repair is still a long way off based on our manual analysis of the generated repaired codes by the learning models.

==> figure_tex/delete_result_fig.tex <==
\begin{figure}[!hb]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \label{fig:R4R_delete}
         \includegraphics[width=\textwidth]{figures/R4R_delete.png}
         \caption{Performance in the Delete class on the Review4Repair dataset}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \label{fig:tufano_delete}
         \includegraphics[width=\textwidth]{figures/tufano_delete.png}
         \caption{Performance in the Delete class on the dataset by Tufano et al.}
     \end{subfigure}
 
    \caption{Performance comparison in the Delete class on both datasets}
    \label{fig:performance comparison on delete class on both dataset}
\end{figure}

==> figure_tex/insert_result_fig.tex <==
\begin{figure}[!hb]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \label{fig:R4R_insert}
         \includegraphics[width=\textwidth]{figures/R4R_insert.png}
         \caption{Performance in the Insert class on the Review4Repair dataset}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \label{fig:tufano_insert}
         \includegraphics[width=\textwidth]{figures/tufano_insert.png}
         \caption{Performance in the Insert class on the dataset by Tufano et al.}
     \end{subfigure}
 
    \caption{Performance comparison in the Insert class on both datasets}
    \label{fig:performance comparison on insert class on both dataset}
\end{figure}

==> figure_tex/update_result_fig.tex <==
\begin{figure}[!ht]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \label{fig:R4R_update}
         \includegraphics[width=\textwidth]{figures/R4R_update.png}
         \caption{Performance in the Update class on the Review4Repair dataset}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \label{fig:tufano_update}
         \includegraphics[width=\textwidth]{figures/tufano_update.png}
         \caption{Performance in the Update class on dataset by Tufano et al.}
     \end{subfigure}
 
    \caption{Performance comparison in the Update class on both datasets}
    \label{fig:performance comparison on update class on both dataset}
\end{figure}

==> listings_tex/prompt_intro.tex <==
% \begin{lstlisting}[caption={Prompt Engineering Example},label={lst:prompt_intro},language=Python]
% Write a python function which can determine if a year is leap year or not

% Certainly! Here's a Python function that determines whether a year is a leap year or not:


% def is_leap_year(year):
%     if year % 4 == 0:
%         if year % 100 == 0:
%             if year % 400 == 0:
%                 return True  # Divisible by 400, so it's a leap year
%             else:
%                 return False  # Divisible by 100 but not 400, not a leap year
%         else:
%             return True  # Divisible by 4 but not 100, so it's a leap year
%     else:
%         return False  # Not divisible by 4, not a leap year

% This function follows the leap year rules:

% If a year is divisible by 4, it might be a leap year.
% If the year is divisible by 100, it might not be a leap year unless it is also divisible by 400.
% If the year is divisible by 400, it is always a leap year.
% If the year is not divisible by 4, it's not a leap year.
% \end{lstlisting}


\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}}
# Write a Python function that can determine if a year is a leap year or not
def is_leap_year(year):
    if year % 4 == 0:
        if year % 100 == 0:
            if year % 400 == 0:
                return True  # Divisible by 400, so it's a leap year
            else:
                return False  # Divisible by 100 but not 400, not a leap year
        else:
            return True  # Divisible by 4 but not 100, so it's a leap year
    else:
        return False  # Not divisible by 4, not a leap year
\end{PythonSourceCode*}
}
\caption{Zero-shot Prompt Engineering Example}\label{lst:prompt_intro}
\end{listing}


==> listings_tex/zero_shot_prompt_example.tex <==
% \begin{lstlisting}[caption={Prompt Example},label={lst:prompt_example},language=Java]
\begin{listing}[H]
{
\begin{JavaSourceCode*}{label=\textcolor{black}{\tiny{prompt\_example.java}}}
Buggy Code:
private FirewallRule findById(List < FirewallRule > collection, String id) {
    FirewallRule result = null;
    for (FirewallRule rule: collection) {
        if (rule.id().equals(id)) { 
            < START > result = rule; < END >
        }
    }
    return result;
}
Review: Just return rule.
Refactor the Buggy Code using the Review without comments.
\end{JavaSourceCode*}
}
\caption{Prompt Example}\label{lst:zero_shot_prompt_example}
\end{listing}
% \end{lstlisting}


==> related_works.tex <==
In recent times, a transformer-based software vulnerability repair method known as VulRepair \cite{VulRepair} has excelled at repairing program vulnerabilities. Essentially, it is a T5-based \cite{RaffelT5} automated software vulnerability repair approach that makes use of the pre-training and Byte Pair Encoding (BPE) components to overcome the technical shortcomings of earlier works \cite{VRepair, feng-etal-2020-codebert} in vulnerability repair tasks. The PL/NL pre-training corpus increases the percentage of accurate predictions for vulnerability repair approaches regardless of the model architecture, demonstrating the significant advantages of adopting pre-training components for vulnerability repair approaches. However, their results degrade significantly when the token size increases. It is worth exploring to see if the use of code review could overcome this limitation to some extent.

==> tables/R4R_dataset_table.tex <==
\begin{table}[h!]
    \centering
    \caption{Overview of Review4Repair Dataset \cite{R4R}}
    \begin{tabular}{ccccc}
        \toprule
        \textbf{\begin{tabular}[c]{@{}c@{}}Dataset\\ Type\end{tabular}} & 
        \textbf{\begin{tabular}[c]{@{}c@{}}Insert\\ Samples\end{tabular}} & 
        \textbf{\begin{tabular}[c]{@{}c@{}}Delete\\ Sample\end{tabular}} & 
        \textbf{\begin{tabular}[c]{@{}c@{}}Update\\ Sample\end{tabular}} & 
        \textbf{\begin{tabular}[c]{@{}c@{}}Total\\ Samples\end{tabular}} \\
        
        \midrule
        Train & 8718 & 4060 & 40420 & 53198 \\
        Test & 222 & 425 & 2308 & 2955 \\
        Evaluation & 247 & 481 & 2228 & 2956 \\
        
        \bottomrule
    \end{tabular}
    \label{tab:R4R-dataset}
    \end{table}
